A Mess of Memory System Benchmarking, Simulation and Application Profiling

The Memory stress (Mess) framework provides a unified view of the memory system benchmarking, simulation and application profiling. The Mess benchmark provides a holistic and detailed memory system characterization. It is based on hundreds of measurements that are represented as a family of bandwidth--latency curves. The benchmark increases the coverage of all the previous tools and leads to new findings in the behavior of the actual and simulated memory systems. We deploy the Mess benchmark to characterize Intel, AMD, IBM, Fujitsu, Amazon and NVIDIA servers with DDR4, DDR5, HBM2 and HBM2E memory. The Mess memory simulator uses bandwidth--latency concept for the memory performance simulation. We integrate Mess with widely-used CPUs simulators enabling modeling of all high-end memory technologies. The Mess simulator is fast, easy to integrate and it closely matches the actual system performance. By design, it enables a quick adoption of new memory technologies in hardware simulators. Finally, the Mess application profiling positions the application in the bandwidth--latency space of the target memory system. This information can be correlated with other application runtime activities and the source code, leading to a better overall understanding of the application's behavior. The current Mess benchmark release covers all major CPU and GPU ISAs, x86, ARM, Power, RISC-V, and NVIDIA's PTX. We also release as open source the ZSim, gem5 and OpenPiton Metro-MPI integrated with the Mess simulator for DDR4, DDR5, Optane, HBM2, HBM2E and CXL memory expanders. The Mess application profiling is already integrated into a suite of production HPC performance analysis tools.

==> 60-future-exploration.tex <==








==> 75-Beyond-mess.tex <==


\rev{The Mess benchmark is also a good starting point for further exploration 
of some important memory aspects that exceed the scope of this study.} 

\rev{\textbf{The memory access pattern} may have a significant impact on the memory system behavior and performance. 
The Mess benchmarks measured the memory access latency with the random-access pointer-chase benchmark
concurrently executed with the multi-process memory traffic generator. 
Each traffic generator process generates sequential addresses, 
but, the memory access pattern is complex due to the traffic interleaving between tens of CPU cores or GPU~SMs. 
Mess traffic generator processes can be easily extended to cover different memory access patterns. 
Some of these patterns are strided access, e.g. targeting a new row-buffer in each operation,  
or the random access, e.g. similar to the Giga Updates Per Second~(GUPS) benchmark~\cite{}. 
The memory access pattern analysis, however, should also consider the translation between the virtual address and the exact data location in memory device: channel, rank, bank-group, bank, row and column.  
This information is proprietary and typically unknown. The same applies to the network on chip and 
memory controller policies that interleave, schedule and prioritize incoming memory requests. 
Although this complex and multidimensional analysis exceeds the scope of this paper, we believe that our study enables
future work on this important memory system aspect. 
A first step in this direction could analyze the impact of the traffic generator access pattern on the the row-buffer hit/miss/empty statistics. This can be monitored with hardware counters available in some of the state-of-the-art architectures~\cite{}.}

\rev{In the current Mess release, \textbf{the memory access latency} is measured with a pointer chase benchmark. 
This approach is selected because it is simple and portable to different actual hardware platforms and simulators.  
Another options would be to use hardware counters available in some of the current architectures~\cite{}. 
For example, Intel processors include Precise Event-Based Sampling~(PEBS) counters for precise measurement of various performance events, including memory access latency~\cite{}. 
The PEBS counters track a sample of all memory access and provide detailed information about each event. 
This could simplify the Mess benchmark because there would be no need 
for a pointer chase. Also, per-process latency monitoring enables detailed analysis 
of the whole memory latency distribution and its tails, e.g. $95^{th}$ or $99^{th}$ percentile, 
which is important in some application domains.  
% 
On the down side, detailed event sampling is platform-specific and typically not well documented. 
It would therefore open a question about the consistency of the measurements between different hardware platforms, especially from different manufacturers. 
% 
Also, but may include some of the system software overheads, so it cannot always provide close-to-the-hardware measurements.  
Overall, we believe that it would be interesting to consider different approaches for memory latency measurements
and the tradeoffs between them. The pointer-chase is simple and portable, but some other options could provide more information with an acceptable loss of generality and user control. } 

 




